Reconciling meta-learning and continual learning with online mixtures of tasks

Learning-to-learn or meta-learning leverages data-driven inductive bias to increase the efficiency of learning on a novel task. This approach encounters difficulty when transfer is not advantageous, for instance, when tasks are considerably dissimilar or change over time. We use the connection between gradient-based meta-learning and hierarchical Bayes to propose a Dirichlet process mixture of hierarchical Bayesian models over the parameters of an arbitrary parametric model such as a neural network. In contrast to consolidating inductive biases into a single set of hyperparameters, our approach of task-dependent hyperparameter selection better handles latent distribution shift, as demonstrated on a set of evolving, image-based, few-shot learning benchmarks.

==> figures/acc_figure.tex <==
\pgfplotsset{
  continuallearning/.style={
    width=\plotwidth, height=\plotheight,
    legend style={font=\tiny},
    label style={font=\bfseries},
    tick label style={font=\footnotesize},
    %xlabel=task index,
  },
}
\begin{figure*}[t]
  \centering
  \input{figures/acc}
  \caption{
    An evolving dataset of \gls{mini} few-shot classification tasks where for the first 
    20k iterations we train on the standard dataset, then switch to a "pencil" effect set of tasks 
    for 10k iterations before finally switching to a "blurred" effect set of tasks until 40k.
    Responsibilities $\gamma^{(\ell)}$ for each cluster are plotted over time.
    Note the  change in responsibilities as the dataset changes at iterations 20k and 30k.
  }
  \label{fig:acc}
  %
\end{figure*}

%\begin{figure*}[t]
%  \centering
%  \input{figures/quad-sine-log-plot}
%  \begin{tikzpicture}[baseline]
%    \caption{
%      (Top)
%      An evolving dataset of quadratic, sinusoidal, and logistic regression tasks.
%      The dataset generates quadratic regression tasks for 700 iterations, then switches to
%      generating sinusoidal regression tasks until iteration 5700 at which point it generates
%      logistic regression tasks.
%      (Below)
%      Note the  change in responsibilities to the second (red) cluster at 700
%      iterations when the sinusoidal tasks are introduced.
%      At 5700 iterations, the logistic tasks (third row) also cause a third (brown) cluster to be
%      introduced.
%    }
%    %
%    \label{fig:continual}
%\end{figure*}

